Cryptographic Verifiability for Voter Registration Systems

Voter registration systems are a critical - and surprisingly understudied - element of most high-stakes elections. Despite a history of targeting by adversaries, relatively little academic work has been done to increase visibility into how voter registration systems keep voters' data secure, accurate, and up to date. Enhancing transparency and verifiability could help election officials and the public detect and mitigate risks to this essential component of electoral processes worldwide. This work introduces cryptographic verifiability for voter registration systems. Based on consultation with diverse expert stakeholders that support elections systems, we precisely define the requirements for cryptographic verifiability in voter registration and systematize the practical challenges that must be overcome for near-term deployment. We then introduce VRLog, the first system to bring strong verifiability to voter registration. VRLog enables election officials to provide a transparent log that (1) allows voters to verify that their registration data has not been tampered with and (2) allows the public to monitor update patterns and database consistency. We also introduce VRLog$^x$, an enhancement to VRLog that offers cryptographic privacy to voter deduplication between jurisdictions - a common maintenance task currently performed in plaintext or using trusted third parties. Our designs rely on standard, efficient cryptographic primitives, and are backward compatible with existing voter registration systems. Finally, we provide an open-source implementation of VRLog and benchmarks to demonstrate that the system is practical - capable of running on low-cost commodity hardware and scaling to support databases the size of the largest U.S. state voter registration systems.

==> figures/fig-maintenance-algo.tex <==
\newcommand{\vt}{\mathsf{voters}}
\newcommand{\p}{\mathsf{proofs}}
\newcommand{\keys}{\mathsf{keys}}
\newcommand{\f}{\mathsf{fields}}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[t]
\begin{algorithm}[H]
\caption{\sysname.\Maintenance}
\begin{algorithmic}
\small
    \Require $\thirdparty, \vrdb, \reg, \voters, \vrdbcols$
    \State run step (1) of \basesys.\Maintenance \Comment{Abort if base module aborts.}\small
    % \State $\vt, \p, \f, \keys \gets (), (), (), ()$
    \State $\vt, \p, \keys \gets (), (), (), ()$
    \For{$i \gets 1$ to $m$}
    \State approved$\gets \false$
    \For{$j \gets 1$ to $n$}
    \If{$\access(\thirdparty, \voter_i, \vrdbcol_j) = 1 \wedge \public(\voter_i, \vrdbcol_j) = 0$}
    \State approved$\gets \true$
    \State \Comment{$e$ is retrieved from $\reg_{\id_{\voter_i}}$}
    \State $\keys \gets \keys \cup \big(\KDF(k_{kdf}, \vrdbcol_j \concat \id_{\voter_i} \concat e)\big)$
    % \State $\f \gets \f \cup (f_{i, j})$
    % \Else \State $\keys, \f \gets \keys \cup (\bot), \f \cup (\bot)$
    \Else \State $\keys \gets (\bot)$
    \EndIf
    \EndFor
    \If{approved}
    \State $\vt \gets \vt \cup (\id_{\voter_i})$
    \State $\p \gets \p \cup \big(\reglookup(\id_{\voter_i})\big)$
    \Else \State $\vt, \p \gets \vt \cup (\bot), \p \cup (\bot)$
    \EndIf
    \EndFor
    \State \Return $(\vt, \p, \keys)$
\end{algorithmic}
\medskip
\hrule
\begin{algorithmic}
\small
    % \Require $\vrdbcols, \regcom, (\vt, \p, \f, \keys)$
    \Require $\vrdbcols, \regcom, (\vt, \p, \keys)$
    \State $\f \gets ()$
    \For{$i \gets 1$ to len$(\vt)$}
    \If{$\vt_i \neq \bot \wedge \regverlookup(\regcom, \vt_i, \p_i) = 0$}
    \State \textbf{abort}
    \EndIf
    \For{$j \gets 1$  to $n$}
    \State $ix \gets i \times n + j$
    \If{$\keys_{ix} \neq \bot\ $}
    \State $\f \gets \f \cup (\Dec_{\keys_{ix}}(\p_{i}[0][j]))$
    \EndIf 
    \EndFor
    \EndFor
    \State run step (2) of \basesys.\Maintenance \Comment{Abort if base module aborts.}
    \State \Return $\f$
\end{algorithmic}
\end{algorithm}
\caption{The main steps involved in interfacing with third parties using \sysname, as run by election officials (top) and third-parties (bottom). Here we show the \Maintenance module as an example, but the steps are general for any interaction.}\label{fig:maintenance-algo}
\vspace{-0.4cm}
\end{figure}




==> figures/fig-modules.tex <==
\usetikzlibrary{shapes,arrows,decorations.pathmorphing,backgrounds,positioning,fit,matrix}
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{voter} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=yellow!30]
\tikzstyle{module} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{vrdb} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=yellow!30]
\tikzstyle{maintainer} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{audit} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=orange!30]


\begin{figure}
\captionsetup[subfigure]{font=footnotesize}
\centering


\captionbox{\label{fig:register-module-diagram} Input and output to the $\Reg$ module. $I$ represents the voters personal information, as indicated by $\pvoterinfo$.}[.47\textwidth]{%
\begin{tikzpicture}[node distance=2.5cm]
\node (voter) [voter] {Voter};
\node (module) [module, right of=voter] {\Reg};
\node (vrdb) [vrdb, right of=module] {VRDB};

\draw [arrow] (voter) -- node[anchor=south] {$I$} (module);
\draw [arrow]  (module) --  node[anchor=south] {$I/\bot$} (vrdb);
\end{tikzpicture}}

\captionbox{\label{fig:maintenance-module-diagram} Main inputs and outputs to the $\Maintenance$ module. $V$ represents a personal identifier for a voter, $I$ their personal information, $I'$ the subset which the maintenance entity (ME) is allowed to access, and $\hat{I}$ the voter's updated information (if any)}[.47\textwidth]{%
\begin{tikzpicture}[node distance=3.5cm]
\node (maintenance) [voter] {ME};
\node (module) [module, right of=maintenance] {\Maintenance};
\node (vrdb) [vrdb, right of=module] {VRDB};

\draw[arrow](module) to[bend right=25] node[below] {\small $(1)\ V$}(vrdb);
\draw[arrow](vrdb) to[bend right=25] node[above] {\small $(2)\ I$} (module);

\draw[arrow] (module) to[bend right=15] node[above] {\small $(3)\ I'$}(maintenance);
\draw[arrow] (maintenance) to[bend right=15] node[below] {\small $(4)\ A$} (module);

\draw [arrow] (module) -- node[anchor=south] {\small $(5)\ \hat{I}$} (vrdb);

\end{tikzpicture}}
\end{figure}


==> figures/fig-priv-algos.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[h]
\begin{algorithm}[H]
\caption{\sysnamepriv.\Query}
\begin{algorithmic}
\small
\Require $\textcolor{red}{P}, \id, \{k_{j,i}\}_{j \in [n], i \in [e]}, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}$
\If{$\regverhistory(\id, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}) = 0$}
\State \textbf{abort}
\EndIf
\For{$i \gets 1$ to $e$}
\For{$j \gets 1$ to $n$}
\If{$\public(\voter, \vrdbcol) = 1$} $f_j = \reg_{\id_i}[j]$
\Else
\State \textcolor{red}{$c', c'' = \reg_{\id_i}[j]$}
\State $f_{j} = \Dec_{k_{j,i}}(c')$ \Comment{Abort if $f_j$ is incorrect.}
\State \textcolor{red}{$\hat{c} = \encode({f_j})$} \Comment{Abort if $\hat{c} \neq c''$.}
\EndIf
\EndFor
\EndFor
\State \Return
\end{algorithmic}
\end{algorithm}
\caption{\Query module of \sysnamepriv. The additions to \sysname are marked in \textcolor{red}{red}. Note that checking that the stored encoding matches the encoded plaintext data may require additional information from election officials (e.g., a secret key), which is left implicit in this algorithm.}\label{fig:priv-query-algo}
\vspace{-0.4cm}
\end{figure}

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

\newcommand{\encodings}{\mathsf{encodings}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[h]
\begin{algorithm}[H]
\caption{\sysnamepriv.\Maintenance}
\begin{algorithmic}
\small
\color{red}
    \Require $P \coloneqq (\encode, \match), \reg^B, \vrdbcols$
    \State $\encodings \gets ()$
    \For{$\id \in \reg^B$}
    \For{$j \gets 1$ to $n$}
    \State $c', c'' = \reg^B_{\id}[j]$
    \State $\encodings \gets c''$
    \EndFor
    \EndFor
    \State $\match(\encodings)$
    \State \Comment{Manually inspect matches, and apply updates as needed.}
    \State \Return
\end{algorithmic}
\end{algorithm}
\caption{The main steps involved in jurisdictions $A$ and $B$ detecting duplicates using \sysnamepriv. This protocol is run by both jurisdictions (shown here for $A$). This module replaces \sysname.\Maintenance.}\label{fig:priv-maintenance-algo}
\vspace{-0.4cm}
\end{figure}

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[h]
\begin{algorithm}[H]
\caption{\sysnamepriv.\Reg}
\begin{algorithmic}
\small
\Require $\vrdb_{\voter} \coloneqq (f_{1}, ..., f_{n}), \textcolor{red}{P \coloneqq (\encode, \match)}, M, e, $
\State run $\basesys.\Reg(\vrdb_{\voter})$ \Comment{Abort if base system aborts.}
\State $\id_\voter \gets F(K_{id}, \vrdb_{\voter})$
\State $r \gets \bot$
\For{$j \gets$ 1 to $n$}
\If{$\public(\voter, \vrdbcol_j) = 1$}
\State $r \gets r \concat f_j$
\Else \State $k_{j} \gets \KDF(K_{kdf}, \id_\voter \concat \vrdbcol_j \concat e)$ 
\State $r \gets r \concat \Enc_{k_{j}}(f_{j}) \textcolor{red}{\concat \encode(f_{j})}$
\EndIf
\EndFor
\State $M \gets M \concat \add$
\State $\pool$.add($\id_\voter, r$)
\State \Return $\id_\voter$
\end{algorithmic}
\end{algorithm}
\caption{The main steps involved in registering new voters using \sysnamepriv. The additions to \sysname are marked in \textcolor{red}{red}.}\label{fig:priv-register-algo}
\vspace{-0.4cm}
\end{figure}

==> figures/fig-priv-query-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[t]
\begin{algorithm}[H]
\caption{\sysnamepriv.\Query}
\begin{algorithmic}
\small
\Require $\textcolor{red}{P}, \id, \{k_{j}\}_{j \in [n]}, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}$
\If{$\regverhistory(\id, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}) = 0$}
\State \textbf{abort}
\EndIf
\For{$i \gets 1$ to $e$}
\For{$j \gets 1$ to $n$}
\If{$\public(\voter, \vrdbcol) = 1$} $f_j = \reg_{\id_i}[j]$
\Else
\State \textcolor{red}{$c', c'' = \reg_{\id_i}[j]$}
\State $f_{j} = \Dec_{k_j}(c')$ \Comment{Abort if $f_j$ is incorrect.}
\State \textcolor{red}{$\hat{c} = \encode({f_j})$} \Comment{Abort if $\hat{c} \neq c''$.}
\EndIf
\EndFor
\EndFor
\State \Return
\end{algorithmic}
\end{algorithm}
\caption{\Query module of \sysnamepriv. The additions to \sysname are marked in \textcolor{red}{red}. Note that checking that the stored encoding matches the encoded plaintext data may require additional information from election officials (e.g., a secret key), which is left implicit in this algorithm.}\label{fig:priv-query-algo}
\vspace{-0.4cm}
\end{figure}

==> figures/fig-priv-register-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[t]
\begin{algorithm}[H]
\caption{\sysnamepriv.\Reg}
\begin{algorithmic}
\small
\Require $\vrdb_{\voter} \coloneqq (f_{1}, ..., f_{n}), \textcolor{red}{P \coloneqq (\encode, \match)}, M, e, $
\State run $\basesys.\Reg(\vrdb_{\voter})$ \Comment{Abort if base system aborts.}
\State $\id_\voter \gets F(K_{id}, \vrdb_{\voter})$
\State $r \gets \bot$
\For{$j \gets$ 1 to $n$}
\If{$\public(\voter, \vrdbcol_j) = 1$}
\State $r \gets r \concat f_j$
\Else \State $k_{j} \gets \KDF(K_{kdf}, \id_\voter \concat \vrdbcol_j \concat e)$ 
\State $r \gets r \concat \Enc_{k_{j}}(f_{j}) \textcolor{red}{\concat \encode(f_{j})}$
\EndIf
\EndFor
\State $M \gets M \concat \add$
\State $\pool$.add($\id_\voter, r$)
\State \Return $\id_\voter$
\end{algorithmic}
\end{algorithm}
\caption{The main steps involved in registering new voters using \sysnamepriv. The additions to \sysname are marked in \textcolor{red}{red}.}\label{fig:priv-register-algo}
\vspace{-0.4cm}
\end{figure}

==> figures/fig-query-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[t]
\begin{algorithm}[H]
\caption{\sysname.\Query}
\begin{algorithmic}
\small
\Require $\id, \{k_{j,i}\}_{j \in [n], i \in [e]}, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}$
\If{$\regverhistory(\id, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}) = 0$}
\State \textbf{abort}
\EndIf
\For{$i \gets 1$ to $e$}
\For{$j \gets 1$ to $n$}
\If{$\public(\voter, \vrdbcol) = 1$} $f_j = \reg_{\id_i}[j]$
\Else\ $f_{j} = \Dec_{k_{j,i}}(\reg_{\id_i}[j])$
\State \Comment{Abort if $f_j$ is incorrect.}
\EndIf
\EndFor
\EndFor
\State \Return
\end{algorithmic}
\end{algorithm}
\caption{Additional \Query module introduced by \sysname.}\label{fig:query-algo}
\vspace{-0.4cm}
\end{figure}

==> figures/fig-register-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[t]
\begin{algorithm}[H]
\caption{\sysname.\Reg}
\begin{algorithmic}
\small
\Require $\vrdb_{\voter} \coloneqq (f_{1}, ..., f_{n}), M, e$
\State run $\basesys.\Reg(\vrdb_{\voter})$ \Comment{Abort if base system aborts.}
\State $\id_\voter \gets F(K_{id}, \vrdb_{\voter})$
\State $r \gets \bot$
\For{$j \gets$ 1 to $n$}
\If{$\public(\voter, \vrdbcol_j) = 1$}
\State $r \gets r \concat f_j$
\Else \State $k_{j,e} \gets \KDF(K_{kdf}, \id_\voter \concat \vrdbcol_j \concat e)$ 
\State $r \gets r \concat \Enc_{k_{j,e}}(f_{j})$
\EndIf
\EndFor
\State $M \gets M \concat \add$
\State $\pool$.add($\id_\voter, r$)
\State \Return $\id_\voter$
\end{algorithmic}
\end{algorithm}
\caption{The main steps involved in registering new voters using \sysname.}\label{fig:register-algo}
\vspace{-0.4cm}
\end{figure}

==> v1/figures/fig-entities-assumptions.tex <==
\begin{table*}
% \resizebox{\linewidth}{!}{
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.1}
    \begin{tabularx}{\textwidth} { 
  >{\raggedright\arraybackslash}p{0.15\textwidth} 
  >{\raggedright\arraybackslash}X 
  >{\raggedright\arraybackslash}X
  >{\raggedright\arraybackslash}X
  >{\raggedright\arraybackslash}X}
      % \begin{tabular}{l l l l} 
     \toprule
      \textbf{Entity} & \textbf{Responsibilities} & \textbf{Mechanisms} & \textbf{Additional Assumptions} & \textbf{Protects Against}\\
     \midrule
     Auditors & Ensure that $\reg$ is updated correctly. & Verify the commitments and update proofs  published to $\bulletin$. & There is at least one honest auditor per epoch. & Split-view attacks from election officials. \\
     Voters &  Ensure the correctness of their personal data in $\reg$. & Request and verify history proofs for their data. & Every epoch is contained in at least one history proof. & Maintenance and oversight entities receiving incorrect data from election officials. \\
     Maintenance entities & Verify the consistency of the data received from election officials. & Verify inclusion proofs with respect to the commitments in $\bulletin$. & \\ 
     % Election officials & \\
     \bottomrule
\end{tabularx}
\caption{Summary of assumptions and responsibilities for each entity in each modified module, and resulting guarantees.}
\vspace{-0.3cm}
\label{fig:entities-assumptions}
% }
\end{table*}

==> v1/figures/fig-modules.tex <==
\usetikzlibrary{shapes,arrows,decorations.pathmorphing,backgrounds,positioning,fit,matrix}
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{voter} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=yellow!30]
\tikzstyle{module} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{vrdb} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=yellow!30]
\tikzstyle{maintainer} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{audit} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=orange!30]


\begin{figure}
\captionsetup[subfigure]{font=footnotesize}
\centering


\captionbox{\label{fig:register-module-diagram} Input and output to the $\Reg$ module. $I$ represents the voters personal information, as indicated by $\pvoterinfo$.}[.47\textwidth]{%
\begin{tikzpicture}[node distance=2.5cm]
\node (voter) [voter] {Voter};
\node (module) [module, right of=voter] {\Reg};
\node (vrdb) [vrdb, right of=module] {VRDB};

\draw [arrow] (voter) -- node[anchor=south] {$I$} (module);
\draw [arrow]  (module) --  node[anchor=south] {$I/\bot$} (vrdb);
\end{tikzpicture}}

\captionbox{\label{fig:maintenance-module-diagram} Main inputs and outputs to the $\Maintenance$ module. $V$ represents a personal identifier for a voter, $I$ their personal information, $I'$ the subset which the maintenance entity (ME) is allowed to access, and $\hat{I}$ the voter's updated information (if any)}[.47\textwidth]{%
\begin{tikzpicture}[node distance=3.5cm]
\node (maintenance) [voter] {ME};
\node (module) [module, right of=maintenance] {\Maintenance};
\node (vrdb) [vrdb, right of=module] {VRDB};

\draw[arrow](module) to[bend right=25] node[below] {\small $(1)\ V$}(vrdb);
\draw[arrow](vrdb) to[bend right=25] node[above] {\small $(2)\ I$} (module);

\draw[arrow] (module) to[bend right=15] node[above] {\small $(3)\ I'$}(maintenance);
\draw[arrow] (maintenance) to[bend right=15] node[below] {\small $(4)\ A$} (module);

\draw [arrow] (module) -- node[anchor=south] {\small $(5)\ \hat{I}$} (vrdb);

\end{tikzpicture}}
\end{figure}


==> v1/figures/fig-priv-query-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[t]
\begin{algorithm}[H]
\caption{\sysnamepriv.\Query}
\begin{algorithmic}
\small
\Require $\textcolor{red}{P}, \id, \{k_{j}\}_{j \in [n]}, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}$
\If{$\regverhistory(\id, \big[(\reg_{\id_i}, t_i)\big]_{i \in [e]}, \Pi^{hist}, [\regcom_i]_{i \in [e]}) = 0$}
\State \textbf{abort}
\EndIf
\For{$i \gets 1$ to $e$}
\For{$j \gets 1$ to $n$}
\If{$\public(\voter, \vrdbcol) = 1$} $f_j = \reg_{\id_i}[j]$
\Else
\State \textcolor{red}{$c', c'' = \reg_{\id_i}[j]$}
\State $f_{j} = \Dec_{k_j}(c')$ \Comment{Abort if $f_j$ is incorrect.}
\State \textcolor{red}{$\hat{c} = \encode({f_j})$} \Comment{Abort if $\hat{c} \neq c''$.}
\EndIf
\EndFor
\EndFor
\State \Return
\end{algorithmic}
\end{algorithm}
\caption{\Query module of \sysnamepriv. The additions to \sysname are marked in \textcolor{red}{red}. Note that checking that the stored encoding matches the encoded plaintext data may require additional information from election officials (e.g., a secret key), which is left implicit in this algorithm.}\label{fig:priv-query-algo}
\vspace{-0.4cm}
\end{figure}

==> v1/figures/fig-priv-register-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{figure}[t]
\begin{algorithm}[H]
\caption{\sysnamepriv.\Reg}
\begin{algorithmic}
\small
\Require $\vrdb_{\voter} \coloneqq (f_{1}, ..., f_{n}), \textcolor{red}{P \coloneqq (\encode, \match)}, M, e, $
\State run $\basesys.\Reg(\vrdb_{\voter})$ \Comment{Abort if base system aborts.}
\State $\id_\voter \gets F(K_{id}, \vrdb_{\voter})$
\State $r \gets \bot$
\For{$j \gets$ 1 to $n$}
\If{$\public(\voter, \vrdbcol_j) = 1$}
\State $r \gets r \concat f_j$
\Else \State $k_{j} \gets \KDF(K_{kdf}, \id_\voter \concat \vrdbcol_j \concat e)$ 
\State $r \gets r \concat \Enc_{k_{j}}(f_{j}) \textcolor{red}{\concat \encode(f_{j})}$
\EndIf
\EndFor
\State $M \gets M \concat \add$
\State $\pool$.add($\id_\voter, r$)
\State \Return $\id_\voter$
\end{algorithmic}
\end{algorithm}
\caption{The main steps involved in registering new voters using \sysnamepriv. The additions to \sysname are marked in \textcolor{red}{red}.}\label{fig:priv-register-algo}
\vspace{-0.4cm}
\end{figure}
